LUNA: A Model-Based Universal Analysis Framework for Large Language Models

Over the past decade, Artificial Intelligence (AI) has had great success recently and is being used in a wide range of academic and industrial fields. More recently, LLMs have made rapid advancements that have propelled AI to a new level, enabling even more diverse applications and industrial domains with intelligence, particularly in areas like software engineering and natural language processing. Nevertheless, a number of emerging trustworthiness concerns and issues exhibited in LLMs have already recently received much attention, without properly solving which the widespread adoption of LLMs could be greatly hindered in practice. The distinctive characteristics of LLMs, such as the self-attention mechanism, extremely large model scale, and autoregressive generation schema, differ from classic AI software based on CNNs and RNNs and present new challenges for quality analysis. Up to the present, it still lacks universal and systematic analysis techniques for LLMs despite the urgent industrial demand. Towards bridging this gap, we initiate an early exploratory study and propose a universal analysis framework for LLMs, LUNA, designed to be general and extensible, to enable versatile analysis of LLMs from multiple quality perspectives in a human-interpretable manner. In particular, we first leverage the data from desired trustworthiness perspectives to construct an abstract model as an auxiliary analysis asset, which is empowered by various abstract model construction methods. To assess the quality of the abstract model, we collect and define a number of evaluation metrics, aiming at both abstract model level and the semantics level. Then, the semantics, which is the degree of satisfaction of the LLM w.r.t. the trustworthiness perspective, is bound to and enriches the abstract model with semantics, which enables more detailed analysis applications for diverse purposes.

==> biosketches.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/DaSong.jpg}}]{Da Song}
is a Ph.D. student at the University of Alberta, Canada. He obtained his B.S. from the University of Minnesota, Twin Cities, USA.
His research interests lie at the intersection of Software Engineering (SE), AI, and Human-Computer Interaction (HCI). He focuses on software testing and analysis for large language models, as well as designing and developing interactive interfaces that can enable more efficient human-in-the-loop AI development.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/xuan.jpg}}]{Xuan Xie}
received the BE degree from Sun Yat-sen University, China, and the master’s degree from Max Planck Institute for Software Systems, Germany. He is currently working toward the PhD degree with the University of Alberta, Canada. His research interests include trustworthiness analysis for large language model, safety analysis of AI-enabled cyber-physical systems, and neural network verification.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/JiayangSong.jpg}}]{Jiayang Song}
is a PhD student at University of Alberta, Canada. He received his B.E. from Western University, Canada and his M.E. from University of Toronto, Canada.
His research topics include testing, analysis, repairing and enhancement of AI systems and their applications to quality assurance of trustworthy AI-enabled cyber-physical systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/DeruiZhu.pdf}}]{Derui Zhu}
is currently a Ph.D. candidate at the Technical University of Munich. His research primarily explores the intersection of security, privacy, and software engineering, with a specific emphasis on trustworthy AI. He focuses particularly on vulnerability analysis and data protection within AI models. Contact him at derui.zhu@tum.de.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/yuheng.jpg}}]{Yuheng Huang}
received a BE degree from the Beijing University of Posts and Telecommunications, China, and a master’s degree from the University of Alberta, Canada. He is currently working toward a PhD degree at the University of Tokyo, Japan. His research interests primarily focus on the quality assurance of AI-enabled complex systems as well as developing interactive interfaces that can enable more efficient human-in-the-loop AI development from Human-Computer Interaction (HCI) perspectives.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/FelixJuefeiXu_journal.jpg}}]{Felix Juefei-Xu} (Member, IEEE) received the Ph.D. degree in Electrical and Computer Engineering from Carnegie Mellon University (CMU), Pittsburgh, PA, USA. Prior to that, he received the M.S. degree in Electrical and Computer Engineering and the M.S. degree in Machine Learning from CMU, and the B.S. degree in Electronic Engineering from Shanghai Jiao Tong University (SJTU), Shanghai, China. Currently, he is a Research Scientist with GenAI at Meta, based in New York City, where he works on robust perception and efficient learning problems in the domain of generative AI. He is also affiliated with New York University as an Adjunct Professor. Previously, he was a Research Scientist with Alibaba Group, based in Sunnyvale, CA. He was the recipient of multiple best and distinguished paper awards, including IJCB 2011, BTAS 2015 and 2016, ASE 2018, and ACCV 2018.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{image/photos/LeiMa.jpeg}}]{Lei Ma}
is currently an associate professor with The University of Tokyo, Japan and University of Alberta, Canada. He was honorably selected as a Canada CIFAR AI Chair and Fellow at Alberta Machine Intelligence Institute (Amii). Previously, he received the B.E. degree from Shanghai Jiao Tong University, China, and the M.E. and Ph.D. degrees from The University of Tokyo, Japan.
His recent research centers around the interdisciplinary fields of software engineering (SE) and trustworthy artificial intelligence with a special focus on the quality, reliability, safety and security aspects of AI Systems.
\end{IEEEbiography}

% that's all folks


==> section/ablation_study.tex <==
\noindent\textbf{Abstract Model Construction Study}

In this section, we aim to investigate the individual contributions of key components in our abstract model construction process to the overall performance and trustworthiness of LLM abstractions. The scope of this analysis includes a range of configurations, providing a comprehensive overview of how different model construction choices affect the trustworthiness and efficacy of LLM abstractions. Specifically, we focus on three critical aspects of model construction: the type of abstract model employed, the role of dimensionality reduction, and the effect of different abstraction/clustering methods combined with discretization strategies.

Through this study, our objectives are twofold:

\begin{itemize}
    \item \textbf{To Quantify the Impact:} By systematically varying each component while keeping others constant, we aim to quantify their individual contributions to the model's ROC AUC performance. This allows us to isolate the effects of each method on the abstract model's effectiveness.

    \item \textbf{To Conduct an Ablation Study:} By incrementally removing or altering components (such as bypassing dimensionality reduction), we evaluate their necessity in the construction process. This ablation aspect helps us understand whether certain steps are critical or if they can be modified or omitted without significant loss in performance.
\end{itemize}
\textbf{Study Component}

\textbf{Abstract Model Type:} The study begins with a comparative analysis between DTMC and HMM to identify which abstract model type best captures the abnormal instances. 

\textbf{Dimensionality Reduction:} Following the selection of an abstract model type, we examine the impact of PCA dimensionality reduction on the model's performance. This component assesses whether reducing the feature space enhances the abstract model's ability to detect abnormal behaviors, and how this process affects the overall trustworthiness assessment.


\textbf{Partition Methods and Discretization: }
The final component evaluates different abstraction and clustering methods, including Grid-based, GMM, and KMeans, alongside their discretization strategies. Given the varying scales of abstract state numbers associated with each method, this analysis explores how these factors influence trustworthiness evaluation.
\\

\noindent\textbf{Setup}

\textbf{Replication for Reliability:}
To enhance the reliability of our findings, we performed five repeated experiments, averaging the results across all trials. This process ensures the consistency and dependability of the outcomes.

\textbf{Abstract Model Type:}
 We used the same settings for abstract model construction in the experiment described in Section 4.2.1 Hyperparameters Settings. We obtained the ROC AUC for all the construction settings, calculated the mean values for the settings that utilize DTMC, and repeated the process for HMM. 

\textbf{PCA Dimension:}
In this part, we systematically increase the PCA dimension to assess its impact on the performance of abstract models. This approach also incorporates an ablation aspect. Specifically, we set the upper bound for the PCA dimension as the hidden dimension of LLM. This approach allows for an ablation study to evaluate the necessity and impact of PCA in the model abstraction process. We start with a PCA dimension of 1, then 10, and incrementally increase it by 10 when the dimension is up to 100. For dimensions greater than 100, we increase it by 100, until it reaches the hidden dimension of the LLM, which means the Dimensionality Reduction is bypassed. In our study, Llama2-7b's hidden dimension is \emph{$4096$}, and CodeLlama-13b's hidden dimension is \emph{$5120$}.
% From the first part of the study, we found that DTMC was better than HMM, so we only used DTMC. The other settings were the same as in Section 4.2.1.

\textbf{Partition Methods and Discretization:}
In our investigation of partition methods, we analyze how various partitioning methods, coupled with differing numbers of abstract states, influence the performance of abstract models. 

For cluster-based methods such as GMM and KMeans, we start with an abstract state count of 5, increase it to 10, and then proceed to increment in steps of 100, starting from 100 up to a maximum of 1000. Beyond this threshold, we escalate the count by a factor of 5. This approach aims to reach a sufficiently high number of abstract states potentially allowing each state to represent a distinct concrete state. 

Similarly, for the Grid-based method, we adopt a parallel approach, with the understanding that the state number in this context is a function of the grid number raised to the power of the PCA dimension. We select 5 as our PCA dimension and start with a grid number of 2, then incrementing it by 5 starting from 5, up to 30. Post this point, we double the grid number until it attains a sufficiently large value. 

This study setting allows us to thoroughly examine the effectiveness of each partition method in model abstraction and carry out a comprehensive ablation study.
\\\\
\textbf{Results}

\textbf{Abstract Model Type:}
\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{image/ablation_model_type.pdf}
\caption{ROC AUC Across Model Type and Datasets.}
\vspace{-5pt}
\label{fig:ablation_model_type}
\end{figure*}

Figure~\ref{fig:ablation_model_type} clearly shows that DTMC outperforms HMM on all tasks w.r.t ROC AUC. The reason why DTMC outperforms HMM is due to its direct transition abstraction approach, which captures the transition dynamics of LLMs more accurately. This can be attributed to the two-level state abstract mechanism, where the hidden states and transitions are fitted on top of the abstract state. On the other hand, the direct transition abstraction of DTMC is more effective in tracing back the transition characteristics of the LLM. This investigation confirms our finding in RQ2.2.

\textbf{PCA Dimension:}
\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{image/ablation_pca.pdf}
\caption{ROC AUC Across PCA Dimension and Datasets.}
\vspace{-5pt}
\label{fig:ablation_pca}
\end{figure*}

In Figure~\ref{fig:ablation_pca}, we observe that the ROC AUC is comparably low only when the PCA Dimension is 1. However, when the PCA Dimension is between 10 to LLM's hidden dimension (bypassing PCA), there is no significant increase or decrease trend in the ROC AUC. This result suggests that the Dimensionality Reduction process can preserve the original information effectively. When we reduce the dimension to 10, the performance is similar to that of the original hidden dimension. 

\textbf{Partition Methods and Discretization:}
\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{image/ablation_discret.pdf}
\caption{ROC AUC Across Partition Methods and Datasets.\xuan{Maybe 1000 and 25000 on the x-axis of GMM and KMeans can be separated more? Now it does not look good.}\da{Fixed}}
\vspace{-5pt}
\label{fig:ablation_partition}
\end{figure*}

In Figure~\ref{fig:ablation_partition}, we can see that the GMM and KMeans cluster-based methods exhibit similar trends. The ROC AUC value rapidly increases with a small number of abstract states, reaches a peak around 1000, and then decreases. On the other hand, the Grid-based method shows a different trend. The ROC AUC value increases with the increase of abstract state numbers. However, after reaching a certain threshold, the ROC AUC value drops rapidly until reaching 0.5.
\\\\
\textbf{Conclusion}

Based on the comparative analysis, it has been found that DTMC performs better than HMM in all tasks. This is attributed to DTMC's superior method of direct transition abstraction, which more accurately captures LLM transition dynamics. The analysis also indicates that even a significant reduction of dimensions, to as few as $10$ dimensions, effectively preserves crucial information and maintains ROC AUC performance. Additionally, the study reveals that while both GMM and KMeans clustering methods show optimal performance at an intermediate number of abstract states, the Grid-based method's performance peaks at a certain threshold before declining. This highlights the nuanced impact of partition methods on model analysis outcomes.

==> section/metrics.tex <==
\section{Applications}
\label{sec:application}

Recent works demonstrate that the abstract model has extensive analysis capability for stateful DNN systems~\cite{du2019deepstellar,zhu2021deepmemory,xie2021rnnrepair}.
Here, to validate the practicality of our constructed abstract models, we mainly apply them into \emph{abnormal behavior detection}, which is a common analysis demand for LLMs~\cite{manakul2023selfcheckgpt,chang2023survey}.
As introduced in Section~\ref{sec:background}, abnormal behavior refers to the unintended expression of LLM, e.g., making up answers or generating biased output~\cite{ouyang2022training,bender2021dangers,kenton2021alignment,santhanam2021rome,huang2021factual}.
To detect such behavior, we leverage the abstract model with the semantics.

In practice, one could design domain-specific detection methods based on different demands and scenarios.
Here, we take OOD sample detection as a concrete example to illustrate how to perform model-based abnormal behavior detection.
Given an output text and the abstract state trace $\{\bar{s_1},\dots, \bar{s_n}\}$, we first compute the corresponding semantics trace $\{\bar{\theta}(\bar{s_1}), \dots, \bar{\theta}(\bar{s_n})\}$.
For OOD detection, we can take the transition probability between two consecutive states, i.e., $s_i$ and $s_{i+1}$, as the semantics $\bar{\theta}(\bar{s_i})$.
Then, we compute a semantics score by taking the mean of the production of the semantics trace value, namely, $\textsc{avg}(\prod\bar{\theta}(\bar{s_i}))$.
Finally, we compare the computed score with a predefined threshold to determine whether the output text is an OOD sample.

We will show more details for the abnormal behavior detection methods in different domains, e.g., truthfulness detection, OOD sample detection, and adversarial attack detection, in the experiment Section~\ref{subsec:rq3}.\xuan{to change}

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{image/rq3_example.pdf}
\caption{RQ3.1: Example of abnormal behavior detection on TruthfulQA. \xuan{risky should be abnormal}, \xuan{"Final Semantics" should be "Semantics Score"}}
\vspace{-10pt}
\label{fig:RQ3_example}
\end{figure}

==> table/baseline_compare.tex <==
\begin{table}[h]
\centering
\caption{The ROC AUC for Trustworthiness Assessment Techniques on TruthfulQA.}
\ifthenelse{\boolean{doublecolumn}}{
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{lllr}
\toprule
    Techniques & Perspectives & LLM & ROC AUC \\
    \midrule
      \tool & \multirow{3}{*}{Hallucination-TruthfulQA} & \multirow{3}{*}{Alpaca-7b} &     \textbf{0.71}  \\
      ITI & &  &  0.63  \\
      SAPLMA & &  &    0.66  \\
    
\bottomrule
\end{tabular}
\vspace{-10pt}
}}{
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{lllr}
\toprule
    Techniques & Perspectives & LLM & ROC AUC \\
    \midrule
      \textbf{\tool} & \multirow{3}{*}{Hallucination-TruthfulQA} & \multirow{3}{*}{Alpaca-7b} &     \textbf{0.71}  \\
      ITI & &  &  0.63  \\
      SAPLMA & &  &    0.66  \\
\bottomrule
\end{tabular}
}}
\label{tab:baseline_compare}
\end{table}

==> table/code_pass.tex <==


\begin{table}[!tb]
    \caption{\textit{Pass@1} rate of different LLMs.}
    \centering
    \small
    \label{tab:code_bench}
     % \resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{lll}
    \toprule
    & \textbf{Humaneval} & \textbf{MBPP} \\
    \midrule
    Incoder & 14.6\% (24/164) & 16.6\% (83/500) \\
    SantaCoder & 1.2\% (2/164) & 8.8\% (44/500) \\
    CodeGen & 21.3\% (35/164) & 28.6\% (143/500) \\
    \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}80.0\% (32/40) & \cellcolor{lightgray}58.4\% (73/125) \\
    \bottomrule
    \end{tabular}
    \vspace{-10pt}
     % }
\end{table}

==> table/code_performance.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Pearson correlation coefficients between uncertainty scores and LLMs' performance on two code generation tasks. The results of VR/VRO are presented as ``{\em cosine distance-based (task-specific distance-based)}.'' Highest correlations from different categories are ranked and highlighted as \colorbox{top1Color}{\textit{top-1}}, \colorbox{top2Color}{\textit{top-2}}, and \colorbox{top3Color}{\textit{top-3}}.}
  \label{tab:evaluation_corrCode}
  \begin{subtable}[h]{\textwidth}
    \setlength{\tabcolsep}{11pt}
    \centering
    % \caption{Single-inference/Sample-based Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{llccccccccc}
        \toprule
        % \rotatebox[origin=c]{90}{rota}}
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{4}{c}{{\bf Single-inference Method}} && \multicolumn{2}{c}{{\bf Sample-based Method}}\\
        \cmidrule{3-6} \cmidrule{8-9}
        && \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} && \textbf{Sample VR} & \textbf{Sample VRO}\\
        \cmidrule{1-6} \cmidrule{8-9}
        \multirow{4}{*}{{HumanEval}} & Codegen  & \toptwohl{-0.346} & -0.206 & -0.289 & -0.156 && -0.344 (\toponehl{-0.428}) & -0.094 (-0.375) \\
        & Incoder & -0.106 & \topthreehl{-0.138} & -0.099 & -0.131  && -0.283 (\toponehl{-0.435}) & -0.031 (-0.351) \\
        & Santacoder & \toptwohl{-0.086} & 0.003 & -0.055 & -0.050 && -0.036 (0.000) & \topthreehl{-0.053} (-0.034) \\
        & GPT3.5 & -0.315 & \toponehl{-0.324} & -0.002 & -0.307 && 0.019 (-0.212) & 0.021 (\toptwohl{-0.226}) \\
        \cellcolor{lightgray}& \cellcolor{lightgray}Codegen & \cellcolor{lightgray}0.069 & \cellcolor{lightgray}\toptwohl{0.175} & \cellcolor{lightgray}0.074 & \cellcolor{lightgray}0.161 && \cellcolor{lightgray}-0.044 (-0.235) &\cellcolor{lightgray} -0.144 (\toponehl{-0.275}) \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}Incoder & \cellcolor{lightgray}\topthreehl{0.165} & \cellcolor{lightgray}0.084 & \cellcolor{lightgray}0.158 & \cellcolor{lightgray}0.087 && \cellcolor{lightgray}-0.084 (-0.267) & \cellcolor{lightgray}-0.204 (\toponehl{-0.271}) \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}Santacoder & \cellcolor{lightgray}\topthreehl{-0.142} & \cellcolor{lightgray}-0.053 & \cellcolor{lightgray}-0.101 & \cellcolor{lightgray}0.093  && \cellcolor{lightgray}-0.042 (-0.113) & \cellcolor{lightgray}-0.078 (\toponehl{-0.282}) \\
        
        \multirow{-4}{*}{\cellcolor{lightgray}{MBPP}}& \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}-0.001 & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}-0.067 & \cellcolor{lightgray}\toptwohl{-0.141} && \cellcolor{lightgray}-0.109 (\toponehl{-0.168}) & \cellcolor{lightgray}-0.063 (-0.149) \\
        \bottomrule
        \end{tabular}
  \end{subtable}
  \vspace{2mm}
  \vfill
  \begin{subtable}[h]{\textwidth}
  \setlength{\tabcolsep}{10.28pt}
  \centering
  % \caption{Perturbation-based Uncertainty Estimation}
  \scriptsize
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{6}{c}{\textbf{Perturbation-based}}\\
        \cmidrule{3-8}
        && \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        \multirow{4}{*}{HumanEval} & Codegen & 0.176 (-0.173) & 0.124 (\topthreehl{-0.231}) & -0.141 (0.103) & -0.153 (-0.011) & 0.103 (-0.094) & 0.063 (-0.189) \\
        
        & Incoder & 0.024 (-0.344) & 0.116 (\toptwohl{-0.346}) & -0.111 (0.225) & -0.121 (0.133) & -0.05 (-0.139) & -0.062 (-0.175) \\

        & Santacoder & -0.059 (0.081) & -0.058 (0.050) & -0.042 (0.021) & 0.002 (-0.020) & -0.068 (\toponehl{0.091}) & -0.065 (0.057) \\
        & GPT3.5 & 0.065 (0.058) & -0.140 (0.116) & -0.041 (\topthreehl{-0.213}) & 0.031 (-0.194) & 0.134 (-0.071) & 0.035 (0.022) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}Codegen & \cellcolor{lightgray}\topthreehl{-0.165} (-0.112) & \cellcolor{lightgray}-0.110 (-0.148) & \cellcolor{lightgray}-0.032 (0.123) & \cellcolor{lightgray}-0.022 (0.104) & \cellcolor{lightgray}-0.164 (-0.072) & \cellcolor{lightgray}-0.102 (-0.093) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}Incoder & \cellcolor{lightgray}-0.188 (-0.245) & \cellcolor{lightgray}-0.196 (-0.217) & \cellcolor{lightgray}-0.173 (-0.014) & \cellcolor{lightgray}-0.161 (-0.080) & \cellcolor{lightgray}\toptwohl{-0.249} (-0.223) & \cellcolor{lightgray}-0.210 (-0.196) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}Santacoder & \cellcolor{lightgray}-0.002 (0.053) & \cellcolor{lightgray}0.064 (-0.026) & \cellcolor{lightgray}0.172 (0.033) & \cellcolor{lightgray}\toptwohl{0.265} (-0.028) & \cellcolor{lightgray}-0.030 (0.058) & \cellcolor{lightgray}0.021 (-0.008) \\
        
        \multirow{-4}{*}{\cellcolor{lightgray}MBPP} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}-0.049 (-0.121) & \cellcolor{lightgray}0.008 (-0.042) & \cellcolor{lightgray}-0.101 (-0.016) & \cellcolor{lightgray}-0.047 (-0.053) & \cellcolor{lightgray}0.046 (\topthreehl{-0.131}) & \cellcolor{lightgray}0.018 (-0.072) \\

        \bottomrule
    \end{tabular}
    \end{subtable}
    \vspace{-10pt}
\end{table*}

==> table/code_performance_old.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Uncertainty Measurement on Code Tasks}
  \begin{subtable}[h]{\textwidth}
    \setlength{\tabcolsep}{11pt}
    \centering
    \caption*{Single-inference Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{lcccc}
        \toprule
        \textbf{Model / Dataset} & \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} \\
        \midrule
        Codegen (Humaneval) & \hl{-0.346} & -0.206 & -0.289 & -0.156 \\
        Incoder (HumanEval) & -0.106 & \hl{-0.138} & -0.099 & -0.131 \\
        Santacoder (HumanEval) & \hl{-0.086} & 0.003 & -0.055 & -0.050 \\
        GPT3.5 (Humaneval) & -0.315 & \hl{-0.324} & -0.002 & -0.307 \\
        \cellcolor{lightgray}Codegen (MBPP) & \cellcolor{lightgray}0.069 & \cellcolor{lightgray}\hl{0.175} & \cellcolor{lightgray}0.074 & \cellcolor{lightgray}0.161 \\
        \cellcolor{lightgray}Incoder (MBPP) & \cellcolor{lightgray}\hl{0.165} & \cellcolor{lightgray}0.084 & \cellcolor{lightgray}0.158 & \cellcolor{lightgray}0.087 \\
        \cellcolor{lightgray}Santacoder (MBPP) & \cellcolor{lightgray}\hl{-0.142} & \cellcolor{lightgray}-0.053 & \cellcolor{lightgray}-0.101 & \cellcolor{lightgray}0.093 \\
        \cellcolor{lightgray}GPT3.5 (MBPP) & \cellcolor{lightgray}-0.001 & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}-0.067 & \cellcolor{lightgray}\hl{-0.141} \\
        \bottomrule
        \end{tabular}
  \end{subtable}
  \vspace{2mm}
  \begin{subtable}[h]{\textwidth}
    \centering
    \caption*{Sample-based Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{lcc}
            \toprule
            \textbf{Model / Dataset} & \textbf{Sample VR} & \textbf{Sample VRO} \\
            \midrule
        Codegen (Humaneval) & -0.344(\hl{-0.428}) & -0.094(-0.375) \\
        Incoder (HumanEval) & -0.283(\hl{-0.435}) & -0.031(-0.351) \\
        Santacoder (HumanEval) & -0.036(0.000) & \hl{-0.053}(-0.034) \\
        GPT3.5 (Humaneval) & 0.019(-0.212) & 0.021(\hl{-0.226}) \\
        \cellcolor{lightgray}Codegen (MBPP) & \cellcolor{lightgray}-0.044(-0.235) &\cellcolor{lightgray} -0.144(\hl{-0.275}) \\
        \cellcolor{lightgray}Incoder (MBPP) & \cellcolor{lightgray}-0.084(-0.267) & \cellcolor{lightgray}-0.204(\hl{-0.271}) \\
        \cellcolor{lightgray}Santacoder (MBPP) & \cellcolor{lightgray}-0.042(-0.113) & \cellcolor{lightgray}-0.078(\hl{-0.282}) \\
        \cellcolor{lightgray}GPT3.5 (MBPP) & \cellcolor{lightgray}-0.109(\hl{-0.168}) & \cellcolor{lightgray}-0.063(-0.149) \\
            \bottomrule
        \end{tabular}
  \end{subtable}
  \vfill
  \begin{subtable}[h]{\textwidth}
  \caption*{Perturbation-based Uncertainty Estimation}
  \scriptsize
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Model / Dataset} & \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        Codegen (Humaneval) & 0.176(-0.173) & 0.124(\hl{-0.231}) & -0.141(0.103) & -0.153(-0.011) & 0.103(-0.094) & 0.063(-0.189) \\
        Incoder (HumanEval) & 0.024(-0.344) & 0.116(\hl{-0.346}) & -0.111(0.225) & -0.121(0.133) & -0.05(-0.139) & -0.062(-0.175) \\
        Santacoder (HumanEval) & -0.059(0.081) & -0.058(0.05) & -0.042(0.021) & 0.002(-0.02) & -0.068(\hl{0.091}) & -0.065(0.057) \\
        GPT3.5 (Humaneval) & 0.065(0.058) & -0.14(0.116) & -0.041(\hl{-0.213}) & 0.031(-0.194) & 0.134(-0.071) & 0.035(0.022) \\
        \cellcolor{lightgray}Codegen (MBPP) & \cellcolor{lightgray}\hl{-0.165}(-0.112) & \cellcolor{lightgray}-0.11(-0.148) & \cellcolor{lightgray}-0.032(0.123) & \cellcolor{lightgray}-0.022(0.104) & \cellcolor{lightgray}-0.164(-0.072) & \cellcolor{lightgray}-0.102(-0.093) \\
        \cellcolor{lightgray}Incoder (MBPP) & \cellcolor{lightgray}-0.188(-0.245) & \cellcolor{lightgray}-0.196(-0.217) & \cellcolor{lightgray}-0.173(-0.014) & \cellcolor{lightgray}-0.161(-0.08) & \cellcolor{lightgray}\hl{-0.249}(-0.223) & \cellcolor{lightgray}-0.21(-0.196) \\
        \cellcolor{lightgray}Santacoder (MBPP) & \cellcolor{lightgray}-0.002(0.053) & \cellcolor{lightgray}0.064(-0.026) & \cellcolor{lightgray}0.172(0.033) & \cellcolor{lightgray}\hl{0.265}(-0.028) & \cellcolor{lightgray}-0.03(0.058) & \cellcolor{lightgray}0.021(-0.008) \\
        \cellcolor{lightgray}GPT3.5 (MBPP) & \cellcolor{lightgray}-0.049(-0.121) & \cellcolor{lightgray}0.008(-0.042) & \cellcolor{lightgray}-0.101(-0.016) & \cellcolor{lightgray}-0.047(-0.053) & \cellcolor{lightgray}0.046(\hl{-0.131}) & \cellcolor{lightgray}0.018(-0.072) \\
        \bottomrule
    \end{tabular}
    \end{subtable}
\end{table*}

==> table/datasets.tex <==
\begin{table}[!tb]
\caption{The collected NLP tasks.}
\centering
\small
\label{tab:tasks}
% \resizebox{0.85\columnwidth}{!}{
\begin{tabular}{llr}
\toprule
\textbf{Dataset} & \textbf{Task Domain}  & \textbf{Size (\#~instances)} \\ \midrule
{\bf TruthfulQA} & Question Answering  & 817 \\
% {\bf Wiki-QA} & Question Answering  & 243 \\
% {\bf CNN/Daily Mail} & Text Summarization  & 11,490 \\
% {\bf WMT 2014}    & Machine Translation & 3,003 \\
% {\bf MBPP} & Code Generation & 500 \\
% {\bf HumanEval} & Code Generation & 164 \\
\bottomrule
\end{tabular}
\vspace{-10pt}
% }
\end{table}

==> table/distance_distribution.tex <==


\begin{table}[!tb]
    \caption{The average distances between code generated by open- and closed-source LLMs.}
    \centering
    \small
    \label{tab:code_dist}
    % \resizebox{0.85\columnwidth}{!}{
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{Perturbation}} &&  \multicolumn{2}{c}{\textbf{Sample}}  \\
    \cmidrule{2-3} \cmidrule{5-6}
    & Open & Closed  && Open & Closed \\
    \midrule
    Cosine & 0.03$\pm$0.02 & 0.03$\pm$0.02  && 0.03$\pm$0.03 & 0.01$\pm$0.01 \\
    CodeBLEU & 0.31$\pm$0.13 & 0.23$\pm$0.12  && 0.51$\pm$0.15 & 0.41$\pm$0.16 \\
    \bottomrule
    \end{tabular}
    \vspace{-10pt}
    % }
    % \vspace{-1mm}
\end{table}

==> table/nlp_performance.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Pearson correlation coefficients between uncertainty scores and LLMs' performance on four NLP tasks. The results of VR/VRO are presented as ``{\em cosine distance-based (task-specific distance-based)}.'' Highest correlations from different categories are ranked and highlighted as \colorbox{top1Color}{\textit{top-1}}, \colorbox{top2Color}{\textit{top-2}}, and \colorbox{top3Color}{\textit{top-3}}.}
  \begin{subtable}[h]{\textwidth}
    \setlength{\tabcolsep}{11pt}
    \centering
    % \caption{Single-inference/Sample-based Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{llccccccccc}
        \toprule
        % \rotatebox[origin=c]{90}{rota}}
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{4}{c}{{\bf Single-inference Method}} && \multicolumn{2}{c}{{\bf Sample-based Method}}\\
        \cmidrule{3-6} \cmidrule{8-9}
        && \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} && \textbf{Sample VR} & \textbf{Sample VRO}\\
        \cmidrule{1-6} \cmidrule{8-9}
        \multirow{4}{*}{{CNN/Daily Mail}} & GPT2  & -0.168 & \topthreehl{-0.198} & -0.036 & -0.158 && -0.325 (-0.091) & \toponehl{-0.510} (-0.189) \\
        & LLaMA & -0.225 & \topthreehl{-0.420} & -0.086 & -0.415  && -0.380 (-0.236) & \toponehl{-0.520} (-0.324) \\
        & GPT3 & \topthreehl{-0.231} & -0.202 & -0.145 & -0.170 && -0.326 (-0.210) & \toponehl{-0.413} (-0.268) \\
        & GPT3.5 & \topthreehl{-0.1187} & -0.1186 & -0.036 & -0.106 && -0.288 (-0.181) & \toptwohl{-0.295} (-0.191) \\
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.0208 & \cellcolor{lightgray}\topthreehl{0.0212} & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}0.014 && \cellcolor{lightgray}-0.333 (-0.168) & \cellcolor{lightgray}\toponehl{-0.567} (-0.335) \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}0.025 & \cellcolor{lightgray}0.030 & \cellcolor{lightgray}\topthreehl{-0.040} & \cellcolor{lightgray}0.007 && \cellcolor{lightgray}-0.257 (-0.136) & \cellcolor{lightgray}\toponehl{-0.655} (-0.396) \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.054 & \cellcolor{lightgray}\toptwohl{-0.207} & \cellcolor{lightgray}-0.016 & \cellcolor{lightgray}-0.172 && \cellcolor{lightgray}-0.275 (-0.136) & \cellcolor{lightgray}\toponehl{-0.359} (-0.164) \\
        
        \multirow{-4}{*}{\cellcolor{lightgray}{Eli5-Category}}& \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}-0.037 & \cellcolor{lightgray}-0.240 & \cellcolor{lightgray}-0.084 & \cellcolor{lightgray}\toponehl{-0.289} && \cellcolor{lightgray}-0.224 (-0.053) & \cellcolor{lightgray}\toptwohl{-0.253} (-0.061) \\
        \multirow{4}{*}{{Wiki-QA}} & GPT2 & -0.110 & -0.003 & \topthreehl{-0.134} & -0.004 && -0.433 (-0.150) & \toponehl{-0.682} (-0.434) \\
        & LLaMA & -0.057 & 0.033 & \topthreehl{-0.099} & -0.020 && -0.347 (-0.260) & \toponehl{-0.598} (-0.468) \\
        & GPT3 & -0.112 & \topthreehl{-0.192} & 0.017 & -0.107 && -0.435 (-0.151) & \toptwohl{-0.449} (-0.164) \\
        & GPT3.5 & -0.051 & \topthreehl{-0.107} & -0.065 & -0.105 && -0.341 (-0.077) & \toponehl{-0.380} (-0.080) \\
        \cellcolor{lightgray}&  \cellcolor{lightgray}GPT2& \cellcolor{lightgray}\topthreehl{0.239} & \cellcolor{lightgray}0.073 & \cellcolor{lightgray}0.282 & \cellcolor{lightgray}0.081 && \cellcolor{lightgray}-0.556 (-0.253) & \cellcolor{lightgray}\toponehl{-0.656} (-0.276) \\
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}-0.044 & \cellcolor{lightgray}-0.153 & \cellcolor{lightgray}-0.060 & \cellcolor{lightgray}\topthreehl{-0.166} && \cellcolor{lightgray}-0.472 (-0.353) & \cellcolor{lightgray}\toponehl{-0.837} (-0.636)\\
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.046 & \cellcolor{lightgray}-0.162 & \cellcolor{lightgray}-0.039 & \cellcolor{lightgray}\topthreehl{-0.176} && \cellcolor{lightgray}-0.228 (-0.275) & \cellcolor{lightgray}-0.235 (\toponehl{-0.306}) \\
        \multirow{-4}{*}{\cellcolor{lightgray}{WMT 2014}} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}0.089 & \cellcolor{lightgray}-0.158 & \cellcolor{lightgray}0.050 & \cellcolor{lightgray}\topthreehl{-0.175} && \cellcolor{lightgray}-0.272 (-0.075) & \cellcolor{lightgray}\toptwohl{-0.282} (-0.045) \\
        \bottomrule
        \end{tabular}
  \end{subtable}
  \vspace{2mm}
  \vfill
  \begin{subtable}[h]{\textwidth}
  \setlength{\tabcolsep}{10.13pt}
  \centering
  % \caption{Perturbation-based Uncertainty Estimation}
  \scriptsize
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{6}{c}{\textbf{Perturbation-based}}\\
        \cmidrule{3-8}
        && \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        \multirow{4}{*}{CNN/Daily Mail} & GPT2 & 0.263 (\toptwohl{0.389}) & 0.143 (0.350) & -0.039 (0.254) & -0.239 (0.292) & 0.065 (0.339) & -0.227 (0.289) \\
        
        & LLaMA & 0.293 (\toptwohl{0.444}) & 0.118 (0.403) & -0.025 (0.329) & -0.315 (0.277) & 0.036 (0.362) & -0.325 (0.294) \\

        & GPT3 & -0.232 (-0.166) & \toptwohl{-0.34} (-0.216) & -0.100 (-0.106) & -0.041 (-0.045) & -0.296 (-0.143) & -0.328 (-0.159) \\
        & GPT3.5 & -0.143 (-0.029) & -0.148 (-0.015) & -0.065 (-0.102) & -0.084 (-0.118) & \toponehl{-0.316} (-0.22) & -0.283 (-0.207) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.453 (-0.173) & \cellcolor{lightgray}-0.456 (-0.182) & \cellcolor{lightgray}-0.243 (-0.107) & \cellcolor{lightgray}-0.241 (-0.13) & \cellcolor{lightgray}\toptwohl{-0.471} (-0.165) & \cellcolor{lightgray}-0.47 (-0.179) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}-0.562 (-0.181) & \cellcolor{lightgray}\toptwohl{-0.565} (-0.196) & \cellcolor{lightgray}-0.406 (-0.150) & \cellcolor{lightgray}-0.434 (-0.160) & \cellcolor{lightgray}-0.541 (-0.168) & \cellcolor{lightgray}-0.537 (-0.181) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.085 (0.128) & \cellcolor{lightgray}-0.112 (0.106) & \cellcolor{lightgray}-0.108 (-0.010) & \cellcolor{lightgray}-0.118 (-0.007) & \cellcolor{lightgray}-0.071 (-0.117) & \cellcolor{lightgray}\topthreehl{-0.15} (-0.143) \\
        
        \multirow{-4}{*}{\cellcolor{lightgray}Eli5-Category} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}-0.033 (-0.042) & \cellcolor{lightgray}-0.050 (-0.034) & \cellcolor{lightgray}-0.005 (-0.067) & \cellcolor{lightgray}0.021 (-0.031) & \cellcolor{lightgray}-0.111 (-0.134) & \cellcolor{lightgray}\topthreehl{-0.118} (-0.110) \\
        
        \multirow{4}{*}{Wiki-QA} & GPT2 & -0.599 (-0.132) & -0.577 (-0.139) & -0.433 (-0.152) & -0.426 (-0.140) & \toptwohl{-0.617} (-0.138) & -0.607 (-0.149) \\
        
        & LLaMA & -0.379 (-0.193) & -0.428 (-0.214) & -0.385 (-0.190) & -0.432 (-0.208) & -0.507 (-0.227) & \toptwohl{-0.527} (-0.239) \\
        & GPT3 & -0.173 (-0.132) & -0.291 (-0.290) & -0.074 (-0.063) & -0.149 (-0.182) & -0.338 (-0.255) & \toponehl{-0.457} (-0.378) \\
        & GPT3.5 & \toptwohl{-0.353} (-0.114) & -0.309 (-0.110) & 0.082 (-0.028) & 0.100 (-0.047) & -0.345 (-0.285) & -0.328 (-0.277) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.231 (-0.005) & \cellcolor{lightgray}\toptwohl{-0.24} (-0.133) & \cellcolor{lightgray}-0.072 (-0.026) & \cellcolor{lightgray}-0.019 (-0.129) & \cellcolor{lightgray}-0.226 (-0.051) & \cellcolor{lightgray}-0.197 (-0.101) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}-0.415 (-0.285) & \cellcolor{lightgray}\toptwohl{-0.417} (-0.307) & \cellcolor{lightgray}-0.208 (0.033) & \cellcolor{lightgray}-0.195 (0.140) & \cellcolor{lightgray}-0.349 (-0.168) & \cellcolor{lightgray}-0.361 (-0.118) \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.166 (-0.073) & \cellcolor{lightgray}-0.169 (-0.097) & \cellcolor{lightgray}-0.071 (-0.133) & \cellcolor{lightgray}-0.077 (-0.130) & \cellcolor{lightgray}-0.22 (-0.094) & \cellcolor{lightgray}\toptwohl{-0.252} (-0.114) \\
        \multirow{-4}{*}{\cellcolor{lightgray}WMT 2014} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}\toponehl{-0.476} (-0.466) & \cellcolor{lightgray}-0.475 (-0.442) & \cellcolor{lightgray}-0.231 (-0.278) & \cellcolor{lightgray}-0.194 (-0.255) & \cellcolor{lightgray}-0.464 (-0.355) & \cellcolor{lightgray}-0.439 (-0.349) \\
        \bottomrule
    \end{tabular}
    \end{subtable}
    \vspace{-10pt}
\label{tab:evaluation_corrNLP}
\end{table*}

==> table/rq2_cluster.tex <==
\begin{table*}
\centering
\caption{Model-wise metrics w.r.t. Partition Method.}
\begin{tabular}{lclccc}
\toprule
Dataset & Metric & Partition Method & Max & Min & Mean \\ 
\midrule
\multirow{18}{*}{advglue++} & \multirow{3}{*}{coverage} & GMM & 1.00 & 1.00 & 1.00 \\ 
& & Grid & 0.99 & 0.93 & 0.93 \\ 
& & KMeans & 1.00 & 1.00 & 1.00 \\ 
& \multirow{3}{*}{perplexity} & GMM & 0.43 & 0.00 & 0.15 \\ 
& & Grid & 0.04 & 0.01 & 0.02 \\ 
& & KMeans & 0.20 & 0.00 & 0.09 \\ 
& \multirow{3}{*}{sensitivity} & GMM & 0.21 & 0.12 & 0.15 \\ 
& & Grid & 0.06 & 0.00 & 0.01 \\ 
& & KMeans & 0.00 & 0.00 & 0.00 \\ 
& \multirow{3}{*}{sink\textunderscore state} & GMM & 0.18 & 0.02 & 0.07 \\ 
& & Grid & 0.18 & 0.00 & 0.05 \\ 
& & KMeans & 0.20 & 0.04 & 0.09 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & GMM & 3.46 & 1.75 & 2.62 \\ 
& & Grid & 1.46 & 0.45 & 1.00 \\ 
& & KMeans & 3.46 & 1.82 & 2.62 \\ 
& \multirow{3}{*}{succinctness} & GMM & 0.01 & 0.00 & 0.00 \\ 
& & Grid & 0.00 & 0.00 & 0.00 \\ 
& & KMeans & 0.01 & 0.00 & 0.00 \\ 
\hline
\multirow{18}{*}{sst2} & \multirow{3}{*}{coverage} & GMM & 1.00 & 1.00 & 1.00 \\ 
& & Grid & 0.75 & 0.16 & 0.46 \\ 
& & KMeans & 1.00 & 1.00 & 1.00 \\ 
& \multirow{3}{*}{perplexity} & GMM & 0.28 & 0.06 & 0.16 \\ 
& & Grid & 0.46 & 0.02 & 0.25 \\ 
& & KMeans & 0.20 & 0.06 & 0.13 \\ 
& \multirow{3}{*}{sensitivity} & GMM & 0.33 & 0.18 & 0.24 \\ 
& & Grid & 0.14 & 0.00 & 0.05 \\ 
& & KMeans & 0.01 & 0.01 & 0.01 \\ 
& \multirow{3}{*}{sink\textunderscore state} & GMM & 0.50 & 0.09 & 0.32 \\ 
& & Grid & 0.32 & 0.00 & 0.06 \\ 
& & KMeans & 0.52 & 0.11 & 0.32 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & GMM & 2.80 & 2.05 & 2.41 \\ 
& & Grid & 1.18 & 0.00 & 0.33 \\ 
& & KMeans & 2.75 & 2.03 & 2.41 \\ 
& \multirow{3}{*}{succinctness} & GMM & 0.15 & 0.05 & 0.10 \\ 
& & Grid & 0.00 & 0.00 & 0.00 \\ 
& & KMeans & 0.15 & 0.05 & 0.10 \\ 
\hline
\multirow{18}{*}{truthful\textunderscore qa} & \multirow{3}{*}{coverage} & GMM & 1.00 & 1.00 & 1.00 \\ 
& & Grid & 0.99 & 0.91 & 0.94 \\ 
& & KMeans & 1.00 & 1.00 & 1.00 \\ 
& \multirow{3}{*}{perplexity} & GMM & 0.04 & 0.00 & 0.03 \\ 
& & Grid & 0.09 & 0.00 & 0.06 \\ 
& & KMeans & 0.07 & 0.01 & 0.03 \\ 
& \multirow{3}{*}{sensitivity} & GMM & 0.03 & 0.02 & 0.03 \\ 
& & Grid & 0.03 & 0.00 & 0.01 \\ 
& & KMeans & 0.01 & 0.00 & 0.00 \\ 
& \multirow{3}{*}{sink\textunderscore state} & GMM & 0.00 & 0.00 & 0.00 \\ 
& & Grid & 0.32 & 0.00 & 0.06 \\ 
& & KMeans & 0.01 & 0.00 & 0.00 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & GMM & 1.79 & 0.10 & 0.80 \\ 
& & Grid & 0.94 & 0.00 & 0.30 \\ 
& & KMeans & 2.08 & 0.03 & 0.73 \\ 
& \multirow{3}{*}{succinctness} & GMM & 0.02 & 0.01 & 0.01 \\ 
& & Grid & 0.00 & 0.00 & 0.00 \\ 
& & KMeans & 0.02 & 0.01 & 0.01 \\ 
\bottomrule
\end{tabular}

\label{tab:statsValues}
\end{table*}


==> table/rq2_model_type.tex <==
\begin{table*}
\centering
\caption{Model-wise metrics w.r.t. Abstract Model Type.}
\begin{tabular}{lclccc}
\toprule
Dataset & Metric & Model Type & Max & Min & Mean \\ 
\midrule
\multirow{12}{*}{advglue++} & \multirow{3}{*}{coverage} & DTMC & 1.00 & 0.93 & 1.00 \\ 
& & HMM & 1.00 & 0.93 & 0.99 \\ 
& \multirow{3}{*}{perplexity} & DTMC & 0.43 & 0.03 & 0.27 \\ 
& & HMM & 0.12 & 0.00 & 0.04 \\ 
& \multirow{3}{*}{sensitivity} & DTMC & 0.20 & 0.00 & 0.07 \\ 
& & HMM & 0.21 & 0.00 & 0.07 \\ 
& \multirow{3}{*}{sink\textunderscore state} & DTMC & 0.05 & 0.00 & 0.04 \\ 
& & HMM & 0.20 & 0.02 & 0.09 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & DTMC & 3.46 & 0.45 & 3.05 \\ 
& & HMM & 2.90 & 0.69 & 2.16 \\ 
& \multirow{3}{*}{succinctness} & DTMC & 0.01 & 0.00 & 0.00 \\ 
& & HMM & 0.01 & 0.00 & 0.00 \\ 
\hline
\multirow{12}{*}{sst2} & \multirow{3}{*}{coverage} & DTMC & 1.00 & 0.16 & 0.68 \\ 
& & HMM & 1.00 & 0.16 & 0.69 \\ 
& \multirow{3}{*}{perplexity} & DTMC & 0.43 & 0.15 & 0.24 \\ 
& & HMM & 0.46 & 0.02 & 0.20 \\ 
& \multirow{3}{*}{sensitivity} & DTMC & 0.32 & 0.00 & 0.08 \\ 
& & HMM & 0.33 & 0.00 & 0.08 \\ 
& \multirow{3}{*}{sink\textunderscore state} & DTMC & 0.26 & 0.00 & 0.08 \\ 
& & HMM & 0.52 & 0.00 & 0.20 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & DTMC & 2.80 & 0.01 & 1.09 \\ 
& & HMM & 2.75 & 0.00 & 1.22 \\ 
& \multirow{3}{*}{succinctness} & DTMC & 0.15 & 0.00 & 0.04 \\ 
& & HMM & 0.15 & 0.00 & 0.04 \\ 
\hline
\multirow{12}{*}{truthful\_qa} & \multirow{3}{*}{coverage} & DTMC & 1.00 & 0.91 & 0.98 \\ 
& & HMM & 1.00 & 0.91 & 0.95 \\ 
& \multirow{3}{*}{perplexity} & DTMC & 0.09 & 0.01 & 0.03 \\ 
& & HMM & 0.08 & 0.00 & 0.05 \\ 
& \multirow{3}{*}{sensitivity} & DTMC & 0.03 & 0.00 & 0.02 \\ 
& & HMM & 0.03 & 0.00 & 0.01 \\ 
& \multirow{3}{*}{sink\textunderscore state} & DTMC & 0.02 & 0.00 & 0.00 \\ 
& & HMM & 0.32 & 0.00 & 0.06 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & DTMC & 1.13 & 0.00 & 0.51 \\ 
& & HMM & 2.08 & 0.01 & 0.56 \\ 
& \multirow{3}{*}{succinctness} & DTMC & 0.02 & 0.00 & 0.01 \\ 
& & HMM & 0.02 & 0.00 & 0.00 \\ 
\bottomrule
\end{tabular}

\label{tab:statsValues}
\end{table*}


==> table/rq2_pca.tex <==
\begin{table*}
\centering
\caption{Model-wise metrics w.r.t. PCA Dimension.}
\begin{tabular}{lclccc}
\toprule
Dataset & Metric & PCA Dim & Max & Min & Mean \\ 
\midrule
\multirow{18}{*}{advglue++} & \multirow{3}{*}{coverage} & 512 & 1.00 & 1.00 & 1.00 \\ 

& & 1024 & 1.00 & 0.99 & 1.00 \\ 
& & 2048 & 1.00 & 0.93 & 0.98 \\ 
& \multirow{3}{*}{perplexity} & 512 & 0.34 & 0.00 & 0.11 \\ 
& & 1024 & 0.41 & 0.00 & 0.12 \\ 
& & 2048 & 0.43 & 0.01 & 0.10 \\ 
& \multirow{3}{*}{sensitivity} & 512 & 0.12 & 0.00 & 0.06 \\ 
& & 1024 & 0.14 & 0.00 & 0.07 \\ 
& & 2048 & 0.21 & 0.00 & 0.09 \\ 
& \multirow{3}{*}{sink\textunderscore state} & 512 & 0.20 & 0.04 & 0.09 \\ 
& & 1024 & 0.17 & 0.02 & 0.08 \\ 
& & 2048 & 0.18 & 0.00 & 0.07 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & 512 & 3.46 & 1.75 & 2.60 \\ 
& & 1024 & 3.46 & 1.21 & 2.57 \\ 
& & 2048 & 3.46 & 0.45 & 2.14 \\ 
& \multirow{3}{*}{succinctness} & 512 & 0.01 & 0.00 & 0.00 \\ 
& & 1024 & 0.01 & 0.00 & 0.00 \\ 
& & 2048 & 0.01 & 0.00 & 0.00 \\ 
\hline
\multirow{18}{*}{sst2} & \multirow{3}{*}{coverage} & 512 & 1.00 & 0.74 & 0.85 \\ 
& & 1024 & 1.00 & 0.47 & 0.70 \\ 
& & 2048 & 1.00 & 0.16 & 0.51 \\ 
& \multirow{3}{*}{perplexity} & 512 & 0.26 & 0.02 & 0.17 \\ 
& & 1024 & 0.28 & 0.06 & 0.18 \\ 
& & 2048 & 0.46 & 0.06 & 0.27 \\ 
& \multirow{3}{*}{sensitivity} & 512 & 0.20 & 0.00 & 0.06 \\ 
& & 1024 & 0.24 & 0.00 & 0.07 \\ 
& & 2048 & 0.33 & 0.00 & 0.12 \\ 
& \multirow{3}{*}{sink\textunderscore state} & 512 & 0.49 & 0.00 & 0.16 \\ 
& & 1024 & 0.52 & 0.00 & 0.17 \\ 
& & 2048 & 0.49 & 0.00 & 0.17 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & 512 & 2.75 & 0.01 & 1.20 \\ 
& & 1024 & 2.75 & 0.01 & 1.17 \\ 
& & 2048 & 2.80 & 0.00 & 1.18 \\ 
& \multirow{3}{*}{succinctness} & 512 & 0.15 & 0.00 & 0.04 \\ 
& & 1024 & 0.15 & 0.00 & 0.04 \\ 
& & 2048 & 0.15 & 0.00 & 0.04 \\ 
\hline
\multirow{18}{*}{truthful\textunderscore qa} & \multirow{3}{*}{coverage} & 512 & 1.00 & 0.99 & 1.00 \\ 
& & 1024 & 1.00 & 0.98 & 0.99 \\ 
& & 2048 & 1.00 & 0.91 & 0.94 \\ 
& \multirow{3}{*}{perplexity} & 512 & 0.04 & 0.01 & 0.03 \\ 
& & 1024 & 0.04 & 0.00 & 0.02 \\ 
& & 2048 & 0.09 & 0.02 & 0.06 \\ 
& \multirow{3}{*}{sensitivity} & 512 & 0.03 & 0.00 & 0.01 \\ 
& & 1024 & 0.03 & 0.00 & 0.01 \\ 
& & 2048 & 0.03 & 0.00 & 0.01 \\ 
& \multirow{3}{*}{sink\textunderscore state} & 512 & 0.32 & 0.00 & 0.07 \\ 
& & 1024 & 0.16 & 0.00 & 0.02 \\ 
& & 2048 & 0.08 & 0.00 & 0.02 \\ 
& \multirow{3}{*}{stationary\textunderscore distribution\textunderscore entropy} & 512 & 1.22 & 0.03 & 0.72 \\ 
& & 1024 & 2.08 & 0.06 & 0.72 \\ 
& & 2048 & 1.02 & 0.00 & 0.35 \\ 
& \multirow{3}{*}{succinctness} & 512 & 0.02 & 0.00 & 0.01 \\ 
& & 1024 & 0.02 & 0.00 & 0.01 \\ 
& & 2048 & 0.02 & 0.00 & 0.00 \\ 
\bottomrule
\end{tabular}
\label{tab:statsValues}
\end{table*}

==> table/rq32_model_coef.tex <==
% \begin{table}[h]
% \centering
% \caption{RQ3.2: Pearson coefficient of model–wise Metrics w.r.t. ROC AUC. SUC: Succinctness, COV: Coverage, SEN: Sensitivity, SS: Sink State, PERP: Perplexity, and SDE: Stationary Distribution Entropy}
% \label{tab:rq32_model_coef}
% \begin{tabular}{lrrrrrr}
% \toprule
% Perspective &  SUC &  COV &  SEN &  SS &  PERP &  SDE \\
% \midrule
% OOD & -0.35 & -0.33 & 0.05 & 0.35 & 0.46 & 0.27 \\
% ADV & -0.38 & -0.33 & 0.04 & 0.34 & 0.46 & 0.27 \\
% Hallucination & 0.02 & 0.06 & 0.20 & 0.04 & -0.08 & -0.44 \\
% \bottomrule
% \end{tabular}
% %\vspace{-10pt}
% \end{table}

\begin{table}[h]
\centering
\caption{RQ3.2: Pearson Coefficient of Model--wise Metrics with respect to ROC AUC for Different Tasks. TQA: TruthfulQA, HE: HumanEval, CSNJ: CodeSearchNet-Java, TCS: TL-CodeSum. A: Alpaca-7b, L: Llama2-7b, C: CodeLlama-13b-Instruct}
\label{tab:model-aucroc-coef}
\ifthenelse{\boolean{doublecolumn}}{
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{llrrrrrr}
\toprule
Perspective & LLM & SUC & COV & SEN & SS & PERP & SDE \\
\midrule
OOD & \multirow{3}{*}{A} & -0.35 & -0.33 & 0.05 & 0.35 & 0.46 & 0.27 \\
Adversarial & & -0.38 & -0.33 & 0.04 & 0.34 & 0.46 & 0.27 \\
Hallucination-TQA & & 0.02 & 0.06 & 0.20 & 0.04 & -0.08 & -0.44 \\ 
\midrule
OOD & \multirow{3}{*}{L} & -0.05 & -0.06 & -0.09 & -0.20 & 0.90 & -0.15 \\
Adversarial & & -0.07 & -0.28 & 0.07 & 0.64 & 0.90 & 0.56 \\
Hallucination-TQA & & 0.45 & 0.37 & 0.11 & 0.28 & 0.63 & 0.11 \\ 
\midrule
Hallucination-HE & \multirow{4}{*}{C} & 0.30 & 0.33 & 0.06 & -0.09 & 0.57 & -0.28 \\
Hallucination-MBPP & & 0.48 & -0.11 & 0.08 & -0.13 & 0.56 & -0.07 \\
Hallucination-CSNJ & & 0.35 & -0.02 & 0.05 & 0.16 & 0.37 & -0.17 \\
Hallucination-TCS & & 0.47 & 0.42 & 0.17 & 0.30 & 0.61 & -0.06 \\
\bottomrule
\end{tabular}
\vspace{-5pt}
}}{
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llrrrrrr}
\toprule
Perspective & LLM & SUC & COV & SEN & SS & PERP & SDE \\
\midrule
OOD & \multirow{3}{*}{A} & -0.35 & -0.33 & 0.05 & 0.35 & 0.46 & 0.27 \\
Adversarial & & -0.38 & -0.33 & 0.04 & 0.34 & 0.46 & 0.27 \\
Hallucination-TQA & & 0.02 & 0.06 & 0.20 & 0.04 & -0.08 & -0.44 \\ 
\midrule
OOD & \multirow{3}{*}{L} & -0.05 & -0.06 & -0.09 & -0.20 & 0.90 & -0.15 \\
Adversarial & & -0.07 & -0.28 & 0.07 & 0.64 & 0.90 & 0.56 \\
Hallucination-TQA & & 0.45 & 0.37 & 0.11 & 0.28 & 0.63 & 0.11 \\ 
\midrule
Hallucination-HE & \multirow{4}{*}{C} & 0.30 & 0.33 & 0.06 & -0.09 & 0.57 & -0.28 \\
Hallucination-MBPP & & 0.48 & -0.11 & 0.08 & -0.13 & 0.56 & -0.07 \\
Hallucination-CSNJ & & 0.35 & -0.02 & 0.05 & 0.16 & 0.37 & -0.17 \\
Hallucination-TCS & & 0.47 & 0.42 & 0.17 & 0.30 & 0.61 & -0.06 \\
\bottomrule
\end{tabular}
}}
\end{table}


==> table/rq32_semantic_coef.tex <==
\begin{table}[h]
\centering
\caption{RQ3.1: Pearson Coefficient of Semantic--wise Metrics with respect to ROC AUC. TQA: TruthfulQA, HE: HumanEval, CSNJ: CodeSearchNet-Java, TCS: TL-CodeSum. A: Alpaca-7b, L: Llama2-7b, C: CodeLlama-13b-Instruct}
\label{tab:semantic-aucroc-coef}
\ifthenelse{\boolean{doublecolumn}}{
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{llrrrrrr}
\toprule
Perspective & LLM & PRE &  ENT &  SL &  NDT &  IVT & NVT \\
\midrule
OOD & \multirow{3}{*}{A} & 0.94 & 0.34 & 0.14 & -0.25 & -0.25 & -0.34 \\
Adversarial & & 0.95 & -0.59 & -0.18 & 0.48 & -0.19 & -0.75 \\
Hallucination-TQA & &  0.81 & -0.07 &  -0.18 &  -0.38 & -0.03 & 0.51 \\ 
\midrule
OOD & \multirow{3}{*}{L} & 0.92 & 0.79 & 0.88 & -0.65 & -0.57 & -0.52 \\
Adversarial & & 0.98 & 0.47 & -0.23 & -0.52 & -0.16 & 0.60 \\
Hallucination-TQA & & 1.00 & 0.52 & 0.69 & -0.30 & -0.46 & -0.36 \\ 
\midrule
Hallucination-HE & \multirow{3}{*}{C} & 1.00 & 0.77 & 0.63 & -0.23 & -0.49 & -0.47 \\
Hallucination-MBPP & & 0.99 & 0.97 & 0.78 & -0.21 & -0.35 & -0.50 \\
Hallucination-CSNJ & & 0.96 & 0.58 & 0.61 & -0.22 & -0.46 & -0.42 \\
Hallucination-TCS & & 0.95 & 0.79 & 0.83 & -0.23 & -0.46 & -0.67 \\

\bottomrule
\end{tabular}
\vspace{-5pt}
}}{
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llrrrrrr}
\toprule
Perspective & LLM & PRE &  ENT &  SL &  NDT &  IVT & NVT \\
\midrule
OOD & \multirow{3}{*}{A} & 0.94 & 0.34 & 0.14 & -0.25 & -0.25 & -0.34 \\
Adversarial & & 0.95 & -0.59 & -0.18 & 0.48 & -0.19 & -0.75 \\
Hallucination-TQA & &  0.81 & -0.07 &  -0.18 &  -0.38 & -0.03 & 0.51 \\ 
\midrule
OOD & \multirow{3}{*}{L} & 0.92 & 0.79 & 0.88 & -0.65 & -0.57 & -0.52 \\
Adversarial & & 0.98 & 0.47 & -0.23 & -0.52 & -0.16 & 0.60 \\
Hallucination-TQA & & 1.00 & 0.52 & 0.69 & -0.30 & -0.46 & -0.36 \\ 
\midrule
Hallucination-HE & \multirow{3}{*}{C} & 1.00 & 0.77 & 0.63 & -0.23 & -0.49 & -0.47 \\
Hallucination-MBPP & & 0.99 & 0.97 & 0.78 & -0.21 & -0.35 & -0.50 \\
Hallucination-CSNJ & & 0.96 & 0.58 & 0.61 & -0.22 & -0.46 & -0.42 \\
Hallucination-TCS & & 0.95 & 0.79 & 0.83 & -0.23 & -0.46 & -0.67 \\

\bottomrule
\end{tabular}
}}
\end{table}

